Scaling Electronic Health Record Foundation Models for Population Health Management

Population health management requires scalable methods to identify individuals at risk of chronic diseases such as cardiovascular conditions and cancer, yet existing approaches rely on fragmented data and resource-intensive screening. We present Scaling Electronic Health Record Foundation Models for Population Health Management, an Electronic Health Record Foundation Model that performs large-scale chronic disease prediction using cross-site longitudinal medical records. We pretrain Scaling Electronic Health Record Foundation Models for Population Health Management on billions of medical events from over 5 million patients across Taiwan and the United States, leveraging a unified code alignment framework to address cross-system heterogeneity, and characterize its scaling behavior via IsoFLOP analysis, training compute-optimal models up to 2.4B parameters. Across 11 chronic disease prediction tasks, Scaling Electronic Health Record Foundation Models for Population Health Management demonstrates strong scaling and generalization, outperforming tree-based models and both general and biomedical language models, achieving over 40% and 70% sensitivity at 99% specificity in U.S. and Taiwan cohorts, respectively. On the EHRShot benchmark, Scaling Electronic Health Record Foundation Models for Population Health Management surpasses prior EHR foundation models trained on in-site data despite substantial distribution shifts, highlighting strong few-shot generalization. Finally, we show that aligned cross-system data provides more effective pretraining signal than duplicating single-site data under data-limited settings, underscoring the importance of alignment for scalable healthcare modeling. Our analysis demonstrates the robustness of EHR-FM in various patient distributions and the benefits of operating in the ICD code space. The code will be open-sourced.

==> Figures/code_alignment.tex <==
\begin{wrapfigure}{tr}{0.3\linewidth}

\centering
\vspace{-0.3cm}
\includegraphics[width=\linewidth]{Figures/code_alignment.pdf}

\caption{Effect of unified coding on NHIRD lung cancer across feature configurations.}
\vspace{-1cm}
\label{fig:code_alignment}

\end{wrapfigure}
